Deterministic Bandwidth of Finite Languages

Bandwidth restricts how far transitions can move under an ordering of the states in an automaton. While every finite language admits a bandwidth-2 NFA representation, the deterministic setting is substantially more restrictive. We investigate the bandwidth of partial DFAs accepting finite languages. We show that bounded bandwidth imposes strong structural restrictions on deterministic representations. We prove that there is an infinite hierarchy of classes of finite languages defined by deterministic bandwidth. As a special case of interest, we consider finite languages accepted by bandwidth-1 partial DFAs, and show that they admit a positional characterization, which yields a polynomial-time decision algorithm. We further study how the minimum DFA bandwidth can be estimated from the structure of the minimal DFA. We derive computable upper and lower bounds based on position-unfolding, and local growth of reachable residual states. These bounds can be computed efficiently and differ by at most a linear factor in the maximum word length. We also present a simple language family where the bounds match exactly.

==> eptcsdata.tex <==
\providecommand{\firstpage}{90}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.7}{10.4204/EPTCS.451.7}}

